Inexact Gradient Projection and Fast Data Driven Compressed Sensing

We study convergence of the iterative projected gradient (IPG) algorithm for arbitrary (possibly nonconvex) sets and when both the gradient and projection oracles are computed approximately. We consider different notions of approximation of which we show that the Progressive Fixed Precision (PFP) and the $(1+\epsilon)$-optimal oracles can achieve the same accuracy as for the exact IPG algorithm. We show that the former scheme is also able to maintain the (linear) rate of convergence of the exact algorithm, under the same embedding assumption. In contrast, the $(1+\epsilon)$-approximate oracle requires a stronger embedding condition, moderate compression ratios and it typically slows down the convergence. We apply our results to accelerate solving a class of data driven compressed sensing problems, where we replace iterative exhaustive searches over large datasets by fast approximate nearest neighbour search strategies based on the cover tree data structure. For datasets with low intrinsic dimensions our proposed algorithm achieves a complexity logarithmic in terms of the dataset population as opposed to the linear complexity of a brute force search. By running several numerical experiments we conclude similar observations as predicted by our theoretical analysis.

==> sections/aconverse1.tex <==
\subsubsection*{A converse example}
Consider a noiseless CS recovery problem where $n =2$, $m=1$ and the sampling matrix (i.e. here a row vector) is 
$A=[1\quad a]$ 
for some parameter $a\in \RR$. Consider the following one-dimensional signal model along the first coordinate:
\eq{
\Cc = \{x\in \RR^2: x(1)\in \RR,\, x(2)=0\}.
}
We have indeed $\vertiii{A}=\sqrt{1+a^2}$. It is easy to verify that both of the embedding constants w.r.t. to $\Cc$ are
\eq{ \mmx=\MM = 1.}
Therefore one can tune $a\rightarrow \infty$ to obtain arbitrary small ratios for $\sqrt{\frac{\mmx}{\vertiii{A}}}={(1+a^2)^{-1/4}}$. 
%$\vertiii{A}$ and $\mmx$ the 

Assume the true signal, the corresponding CS measurement,  and the initialization point are
\eq{
x^\gt=[1 \quad 0]^T,\quad y=Ax^\gt=1 \qandq x^0=[0 \quad 0]^T.
}
%and the initialization point $x^0=(0,0)^T$. 
Consider an adversarial $(1+\epsilon)$-approximate projection oracle which performs the following step for any given $x\in \RR^2$: \marginpar{\todo{verify + this part modified $\epsilon$}}
\eq{
		\pp_\Cc^{\epsilon}(x) := [x(1)+\epsilon x(2) \quad 0]^T.
	}
For simplicity we assume no errors on the gradient step. 	
By setting $\mu=1/\beta=1$, the corresponding inexact IPG updates as 
\eq{	
	x^k(1)= 1+\epsilon a \left(1-x^{k-1}(1)\right)  
}
and only along the first dimension (we note that due to the choice of oracle $x^k(2)=0, \forall k$). Therefore we have
\eq{	
	x^k(1)= 1-\left(-\epsilon a\right)^k.
}
which requires $\epsilon<a^{-1}$ for convergence, and it diverges otherwise. As we can see for $a\rightarrow \infty$  %(i.e. where $A$ becomes extremely unstable w.r.t. sampling the first dimension)
i.e. small ratio $\sqrt{\frac{\mmx}{\vertiii{A}}}$, 
the range of admissible $\epsilon$ shrinks, regardless of the fact that the restricted embedding $\mmx=\MM$ exhibits a  perfect isometry; which is an ideal situation for solving CS (i.e. in this case an exact IPG takes only one iteration to converge).

==> sections/covertree1.tex <==
\subsection{Cover tree for fast NN}
With data driven CS formalism and discretization of the model  %$\Cc = \prod_{i=1}^N \Mb$, 
the projection step of IPG reduces to searching the nearest atom in each of the product spaces, however in a potentially very large size $d$ dictionary. 
A very well-established approach to overcome the complexity of an exhaustive nearest neighbour search on a large dataset consists of hierarchically partitioning the solution space and forming a \emph{tree} whose nodes representing those partitions, and then using branch-and-bound methods on the resulting tree for a fast Approximate NN (ANN) search with $o(d)$ complexity e.g. see~\cite{Navigating,beygelzimer2006cover}.

In this regard, we address the computational shortcoming of the projection step in the exact IPG by preprocessing $\widetilde \Cc$ and form a \emph{cover tree} structure suitable for fast ANN searches \cite{beygelzimer2006cover}. Cover tree is a levelled tree whose nodes at different scales form  covering nets for $\widetilde \Cc$ at multiple resolutions (i.e., coarse-to-fine dyadic coverage levels). %This structure hierarchically partitions the metric space and enables using branch-and-bound methods for fast NN search. 
While the tree construction is blind to the explicit structure of data, several key growth properties such as the tree's explicit depth, the number of children per node, and importantly the overall NN complexity are characterized by the intrinsic dimension $\dim(\widetilde \Cc)$ of the model (which in practice  is a small number e.g. when $\widetilde \Cc$ uniformly samples of a low dimensional manifold).





Let $\Tt_\Mb$ denotes a cover tree defined in order to arrange dataset $\Mb$.  %Cover tree is a leveled tree with multiple scales $i=0,\dots,L_{\max}$ where its nodes are associated with data points in  $\Mb$. 
We denote by $\Ss_i$ the set of nodes appear at scale $i=0,\dots,L_{\max}$.
The lowest scale $i=0$ correspond to the root $\Ss_0$ which is a point covering all data. We denote by $\sigma:=\max_{q\in\Mb}\dist(\Ss_0,q)$ the maximum coverage i.e. the maximum distance between the root and any other node on the tree. As we descend down the tree (i.e. incrementing the scale) the nodes present at higher scales cover their descendants at finer resolutions. More precisely, a cover tree structure must have the following  three properties:
% node $i$ denoted by $\Nn_{ji}$ represents a section of the space denoted by$\Ss_{ji}$. Nodes and represented partitions must satisfy the following three properties.
\begin{enumerate}
	\item Nesting: $\Ss_i \subseteq \Ss_{i+1}$, 
	that is once a point $p$ appears as a node in $\Ss_i$, then every lower level in the tree has a node associated with $p$.
	\item Covering: every node $q\in \Ss_{i+1}$ has a parent node  $p\in \Ss_{i}$, where $\dist(p,q)\leq \sigma2^{-i} $. As a result, covering becomes finer at higher scales in a dyadic fashion. 
	%and For every $p\in \Ss_{i−1}$, there exists
	%a q 2 Ci such that d(p, q) < 2i and the node in
	%level i associated with q is a parent of the node
	%in level i − 1 associated with p.
	
	\item Separation: nodes belonging to the same scale are separated by a minimal distance which dyadically shrinks at higher scales i.e. $\forall q,q'\in\Ss_i$ we have $\dist(q,q')>\sigma2^{-i}$.   
\end{enumerate}  
Each node $p$ also keeps the maximum distance to its descendants denoted by
\eq{maxdist(q):= \max_{q'\in \text{descendant}(q)} \dist(q,q'),
}
which will be useful for the fast NN search.  Note that one might decide to avoid saving $maxdist$ values and use the following upper bound instead.


{\lem{\label{lem:maxdist}For any $q\in \Ss_i$ and due to the covering property we have:
\begin{align}\label{eq:maxdist}
maxdist(q) \leq \sigma \left( 2^{-i}+2^{-i-1}	+ 2^{-i-2}+\dots \right)
< \sigma 2^{-i+1}.
\end{align}
}}

Depth of the \emph{implicit} cover tree (constructed w.r.t. the three constraints above) might grow very large for arbitrary datasets. Indeed we can easily verify that $L_{\max}\leq \log(\Delta(\Mb))$, where 
\eq{
	\Delta(\Mb):= \frac{\max_{p,q \in \Mb}\dist(p,q)}{\min_{p\neq q \in \Mb}\dist(p,q)}.
}
is the aspect ratio of $\Mb$. In practice however we only keep one copy of the nodes which do not have either parent or a child other than themselves. This \emph{explicit} representation efficiently reduces the required storage space to $O(n)$. 

\begin{algorithm}[t]
	\label{alg:findNN}
	\SetAlgoLined
	$Q_0 = \{\Ss_0\}$, where $\Ss_0$ is the root of $\Tt_{\Mb}$\\
	$d_{\min}=\norm{p-q_c}$\\
	$i=0$\\
	\While{$i<L_{\max}$ \& $! \textbf{stoppage}(\gamma)$}
	{
		$Q=\left\{\text{children}(q):\, q\in Q_i \right\} $\\
		$q^* = \argmin_{q\in Q} \norm{p-q}$, \quad $d = \norm{p-q^*}$ \\
		\If{$d<d_{\min}$}{$d_{\min}=d, \quad q_c=q^*$}
		$Q_{i+1} = \left\{q\in Q: \norm{p-q}\leq d_{\min} + maxdist(q) \right\}$\\
		$i  = i+1$\\
	}	
	\Return $q_c$\\%=\argmin_{q\in Q_{L_{\max}}} \norm{p-q}$\;
	\caption{\label{alg:NN} \textbf{ANN}(cover tree $\Tt_\Mb$, query point $p$, current estimate $q_c \in \Mb$, accuracy parameter $\gamma$)}
\end{algorithm}

Algorithm \ref{alg:NN} details the procedure for approximate nearest neighbour (ANN) search on a given cover tree. 
In short, we iteratively traverse down the cover tree and at each scale we populate the set of candidates $Q_i$ with nodes that can be ancestors of the closest NN point and discard others (this refinement uses the triangular inequality and the lower bound on the distance of the grandchildren of $Q$ to $p$, based on  $maxdist(q)$). In the next iteration, children of these candidates are similarly refined and added to the updated candidate set $Q_{i+1}$. At the finest scale (before stoppage) we search the whole set of final candidates and report an ANN point. Not that at each scale we only compute distances for non self-parent nodes (we pass, without computation, distance information of the self-parent children to finer scales).

Three stoppage criteria can be adopted:
\begin{itemize}
	\item \textbf{Fixed-precision:} that is traversing down the tree up to a scale for which the covering resolution falls below a threshold $\gamma$. Given the knowledge of $maxdist$ (or the bound in Lemma \ref{lem:maxdist}) we stop the search when
	%the stoppage can be refined to 
	\eq{ \max_{q\in Q_i} \{maxdist(q)\} < \gamma. }
	 This is similar as performing exact NN searches on a truncated (low-resolution) cover tree. 
	\item \textbf{PFP decaying at rate $r$:} as defined in Corollary \ref{cor:decay}. For this case we perform the stoppage procedure above for an updating accuracy parameter 
	\eq{ 
		\gamma := \nup^k =r^k
		}
	that geometrically decays at a certain rate $r<1$ through the iterations.
	\item \textbf{Relative $\epsilon$-ANN:} It is proposed by \nref KL [Nav.Nets] and Beygelzeimer et al. [CT] that if for a parameter $\gamma=\epsilon$ the search stops as soon as having
	\eq{(1+\frac{1}{\epsilon-1})\sigma2^{-i+1}\leq \argmin_{q\in Q_i} \norm{p-q}
		}
	then we achieve a relative accuracy of type defined by \eqref{eq:eproj}.  
\end{itemize}


==> sections/intro.tex <==
\section{Introduction}
We consider solving the following optimization:
\eql{\label{eq:p1}
	\min_{x\in \Cc} f(x).
	}
We assume:
\begin{description}
\item [A1] Problem \eqref{eq:p1} has solution(s) $x^*$.	
\item [A2]The constraint set $\Cc\in \RR^n$ is closed\footnote{Closeness of $\Cc$ and a lower bound on $f$ implies the existence of a minimum $x^*$ for \eqref{eq:p1}. However we one can drop the closeness and use approximation, see \cite{Blumen}.} and has a well-defined Euclidean projection $\pp_\Cc:\RR^n\rightarrow \Cc$. %that is well defined $\forall x\in \RR^n$ w.r.t. the Euclidean metric. 
\item [A3] The loss function $f(x):\RR^n\rightarrow \RR$ is bounded below, and has a well-defined gradient $\nabla f(x), \forall x\in \Cc$.
\item [A4] $f$ satisfies the Restricted Lipschitz Smoothness (RLS): $\forall x,x'\in \Cc$ it holds 
\eq{ f(x')-f(x) \leq \langle x'-x,\nabla f(x)\rangle + \frac{\MM}{2} \norm{x'-x}^2,}
where $M>0$ is the smallest constant satisfies the inequality above.
%\item [A4]  $f$ satisfies the Restricted Strong Convexity (RSC) for an (global) optimal point $x^*$ of \eqref{eq:p1} i.e., $\forall x\in \Cc$ it holds:
%\eq{ f(x^*)-f(x) \geq \langle x^*-x,f'(x)\rangle + \frac{\mm_{x^*}}{2} \norm{x-x^*}^2.}
\item [A5]  $f$ satisfies the Restricted Strong Convexity (RSC) for a non empty set $\Omega\in \Cc$: for each $x^\rsc\in\Omega$ it holds
\begin{align*} 
f(x^\rsc)-f(x) &\geq \langle x^\rsc -x,\nabla f(x)\rangle + \frac{\mm_{x^\rsc}}{2} \norm{x^\rsc-x}^2,\\
f(x)- f(x^\rsc) &\geq \langle x-x^\rsc,\nabla f(x^\rsc)\rangle + \frac{\mm_{x^\rsc}}{2} \norm{x^\rsc-x}^2.
\end{align*}
\end{description}





\section{Exact Iterative Projected Gradient}
First order methods in form of iterative projected gradient (IPG) are very popular to solve problem \eqref{eq:p1}. For positive integers $k$ and a well-chosen step size $\mu$, IPG iterates as follows:
\eql{\label{eq:IP}x^{k+1} = \pp_\Cc(x^k-\mu \nabla f(x^k)).}
We do not make a particular assumption on the initialization of \eqref{eq:IP} and we set $x^0=0$ throughout.
%they can handle complex sets $\Cc$ (as long as A1 holds). They are suitable for high dimensional inference tasks: their convergence is almost independent of dimension, cost per iteration is scalable with data size, they can be redesigned as stochastic descend with cheap cost per iteration.  

{\thm{\label{th:exactf} Assume (\textbf{A1-A5}) and $\MM< 2\mm$. Set the step size $(2\mm)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:IP} obeys the following bounds:
%\eq{
%	\norm{x^{k+1}-x'}\leq \left(\sqrt{\frac{1}{\mu \mm} -1}\right)^k \norm{x^0-x'} + \frac{2\norm{\nabla f(x')}}{m(1-(\sqrt{\frac{1}{\mu \mm} -1})}
%	}
\begin{itemize}
	\item For any $x^\rsc\in \Omega$ and positive integer $k$
	\eq{
	\norm{x^{k}-x^\rsc}\leq \rho^k \norm{x^\rsc} + \frac{2}{m(1-\rho)}\norm{\nabla f(x^\rsc)},
} 
where $\rho=\sqrt{\frac{1}{\mu \mm} -1}$.

\item  After a finite number $k\geq K$ of iterations 
\eq{
	\norm{x^{k}-x^*}\leq %\rho^k \norm{x^0-x'} +
 \frac{6-2\rho}{m(1-\rho)} \norm{\nabla f(x^\rsc_{\min})}.
 }
Where,
\begin{align*}
&x^\rsc_{\min}\in \argmin_{x^\rsc\in \Omega}\norm{\nabla f(x^\rsc)},\\
&K=\left\lceil\log_\rho\left( \frac{2\norm{\nabla f(x^\rsc_{\min})}}{m(1-\rho) \norm{x^\rsc_{\min}}}\right)\right\rceil,
\end{align*} 
and $x^*$ is a global solution of \eqref{eq:p1}.

\end{itemize}

		}}








\section{Inexact Iterative Projected Gradient}
In this section we show that IPG is robust against deterministic (worst case) errors. Moreover, we show that for certain decaying approximation errors, IPG solution maintain  the same accuracy as for the approximation-free (exact IPG) case.
\subsection{Absolute Approximation Errors}
inIPG iterates as follows:
\eql{\label{eq:inIP} x^{k+1} = \pp_\Cc\left(x^k-\mu( \nabla f(x^k) + \eg^k)\right) + \ep^k,}
where $\ep^k,\eg^k\in \RR^n$ account for (approximation) errors in calculating the projection and gradient steps respectively, and they both assumed to have bounded norms 
\eq{\norm{\ep^k}\leq \nup^k \qandq \norm{\eg^k}\leq \nug^k.}
Note that in this part we assume neither errors $\ep^k,\eg^k$ depend to the previous solutions and thus we refer to them as the \emph{absolute} approximation errors.  


{\thm{\label{th:inexact1}Assume (\textbf{A1-A5}) and $\MM< 2\mm$. Set the step size $(2\mm)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP} obeys the following bounds:
\begin{itemize}
	\item For any $x^\rsc\in \Omega$ and positive integer $k$
	\eq{
		\norm{x^{k}-x^\rsc}\leq  \rho^k \left(\norm{x^\rsc}+\sum_{i=1}^k \rho^{-i} \nut^i \right)+ \frac{2}{m(1-\rho)}\norm{\nabla f(x^\rsc)}
	} 
	%where, \eq{\nut^i=%\sum_{i=1}^k \rho^{-i}
	% \left(\frac{2\nug^i}{m} + \sqrt{\frac{\nup^i}{\mu m}}\right).}
	
	\item The distance to $x^*$ the global solution of \eqref{eq:p1}
	\eq{
		\norm{x^{k}-x^*}\leq  \rho^k \left(\norm{x^\rsc}+\sum_{i=1}^k \rho^{-i} \nut^i \right)+ \frac{2(2-\rho)}{m(1-\rho)}\norm{\nabla f(x^\rsc)}
	} 
	where, \eq{\nut^i=%\sum_{i=1}^k \rho^{-i}
		\frac{2\nug^i}{m} + \sqrt{\frac{\nup^i}{\mu m}},}
\end{itemize}		
and $\rho$ is the same as in Theorem \ref{th:exactf}.		
	}
}

We achieve a linear convergence 
%(up to a tolerance level determined by $\norm{\nabla f(x^\rsc_{\min})}$)
 as long as $\nut^k$ geometrically decays to zero. 	
The following corollary makes this statement explicit:

{\cor{Assume $\nut^k= O(r^k)$ for some $0<r<1$. We have 
		%After a finite number $k\geq K$ of iterations 
		\eq{
			\norm{x^{k}-x^*}\leq %\rho^k \norm{x^0-x'} +
			\frac{4-2\rho}{m(1-\rho)} \norm{\nabla f(x^\rsc_{\min})}+ O({\bar \rho}^k), 
		}
		where $\rho$ and $x^\rsc_{\min}$ are the same as in Theorem \ref{th:exactf},
		\begin{align*}
		%&x^\rsc_{\min}\in \argmin_{x^\rsc\in \Omega}\norm{\nabla f(x^\rsc)},\\
		%&K=\left\lceil\log\left( \frac{2\norm{\nabla f(x^\rsc_{\min})}}{m(1-\rho) \norm{x^\rsc_{\min}}}\right)/\log(\bar \rho)\right\rceil,\\
		\bar \rho = \choice{\max(\rho,r) \qforq r\neq\rho \\
		                	r+\delta     \qforq r=\rho}
		\end{align*}
and any small $\delta>0$.	
		}
	}



\subsection{$(1+\epsilon)$-Approximate Projection}
$\pp\epsilon$


\section{Constrained Least squares} 
Here $f(x):= \frac{1}{2}\norm{y-Ax}^2$. Assumptions \textbf{A4-A5} can be equivalently summarized into the following property:
{\defn{[A6] $A$ is bi-Lipschitz w.r.t. $\Cc$ and $x_0\in \Cc$ if the two following inequalities hold:
		\begin{align*}
		&\norm{A(x-x')}^2\leq M \norm{x-x'}^2 \quad \forall x,x'\in \Cc\\
		&\norm{A(x-x_0)}^2 \geq m_{x_0} \norm{x-x_0}^2 \quad \forall x\in \Cc.
		\end{align*}				
		}}
\subsection{Absolute Approximation Errors}		
{\thm{\label{th:inexactLS1}Assume (\textbf{A1-A2, A6}) and $\MM< 2\mm$. Set the step size $(2\mm)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP} obeys the following bounds:
\eq{
\norm{x^{k}-x_0}\leq  \rho^k \left(\norm{x^\rsc}+\sum_{i=1}^k \rho^{-i} \nut^i \right)+ \frac{2\sqrt{M}}{m(1-\rho)}w
	}
where $w=\norm{y-Ax_0}$, $\rho$ and $\nut^i$ are the same as in Theorem \ref{th:inexact1}.
}} 


\subsection{$(1+\epsilon)$-Approximate Projection}

{\thm{\label{th:inexactLS2}Assume (\textbf{A1-A2, A6}). Let
	\eq{\frac{\norm{A}}{\sqrt m}h(\epsilon)\leq \theta<1 \qandq \MM< (2+\theta^2-2\theta) \mm.} Set the step size $\left((2+\theta^2-2\theta) \mm\right)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP} obeys the following bounds:
		\eq{
			\norm{x^{k}-x_0}\leq  \rho^k \left(\norm{x^\rsc}+\sum_{i=1}^k \rho^{-i} \nut^i \right)+ \left(\frac{ 2\frac{\sqrt{M}}{m}+\sqrt{\frac{\mu}{m}}h(\epsilon)}{1-\rho}\right)w
		}
		where 
		\begin{align*}
		&\rho=\sqrt{\frac{1}{\mu \mm} -1}+\frac{\norm{A}}{\sqrt{m}} h(\epsilon)\\
		&\nut^i= \left(\frac{1}{m}+\sqrt{\frac{\mu}{m}}h(\epsilon)\right)\nug^i
		\end{align*}
		
		and $w=\norm{y-Ax_0}$.
	}} 

==> sections/introLS1.tex <==
\section{Introduction}
Signal inference under limited and noisy observations is a major line of research in signal processing, machine learning and statistics\todo{and it has a wide application ranging from biomedical imaging, astrophysics, remote sensing  to data mining..ask mike to complete}. Exploring the structure of signals is proven to significantly help with an accurate inference since natural datasets often have limited degrees of freedom as compared to their original ambient dimensionality. This fact has been invoked in Compressed sensing (CS)  literature by adopting efficient signal models to achieve accurate signal reconstruction given near-minimal number of measurements i.e. much smaller than the signal original dimension (see \cite{DonohoCS, CRT:CS,Tropp:SOMP1,Candes:EMC,BW:manifold,modelbasedCS} and e.g. \cite{RichCSreview} for an overview on different CS models).
\todo{This for instance in sensory scenarios such as in MRI, video, high resHSI saves a lot of energy cost time...} 
%Compressed sensing (CS) algorithms adopt efficient signal models to achieve accurate reconstruction given small number of measurements. 
CS consists of a linear sampling protocol:
\eql{
	\label{eq:CSsampling}
	y \approx Ax^\gt,
}
where a linear mapping $A$ samples a $m$-dimensional vector $y$ of noisy measurements from a ground truth signal $x^\gt$ which typically lives in a high ambient dimension $n\gg m$. Natural signals often have efficiently compact representations using nonlinear models such as low dimensional smooth manifolds, lowrank matrices or the Union of Subspaces (UoS) that itself includes sparse (unstructured) or structured sparse (e.g. group, tree or analysis sparsity) representations in properly chosen orthobases or redundant dictionaries\nref.
%An efficient CS scheme incorporates such non-linearity into the reconstruction phase to achieve robustness and better compression rates. 
CS reconstruction algorithms for estimating $x^\gt$ from $y$ are in general more computationally complex (as opposed to the CS simple linear acquisition) as they require to handle  mostly non-linear and complicated models. % signal models.  
 A proper model should be carefully chosen in order to efficiently promote the low-dimensional structure of signal meanwhile not bringing a huge computational burden to the reconstruction algorithm.

Consider the following constrained least square problem for CS reconstruction:
\eql{\label{eq:p1}
	\min_{x\in \Cc'} \{f(x):= \frac{1}{2}\norm{y-Ax}^2\},
}
where, the constraint set $\Cc'\in \RR^n$ represents the signal model. First order algorithms in the form of projected Landweber iteration a.k.a. iterative projected gradient (IPG) descend or Forward-Backward are very popular for solving \eqref{eq:p1}. 
% in both convex and nonconvex settings. 
%In this case IPG iterates between calculating the gradient and projection onto the model 
% i.e. for positive integers $k$ and an initialization $x^0$ we have:
%\eql{\label{eq:IP}x^{k} = \pp_\Cc'\left(x^{k-1}-\mu \nabla f(x^{k-1})\right) }
%where, $\nabla f(x)=A^T(Ax-y)$. It has been shown that under certain conditions and for a well chosen step size $\mu$ IPG converges to a solution of \eqref{eq:p1}.
%We do not make a particular assumption on the initialization of \eqref{eq:IP} and we set $x^0=0$ throughout. 
Interesting features of IPG include flexibility of handling various and often complicated models, e.g. $\Cc'$ might be convex, nonconvex or/and semi-algebraic such as sparsity or rank constraints which for the latter IPG deals with solving a combinatorial problem.
%, as long as local oracles gradient (the forward model) and Euclidean projection onto $\Cc' $ are available. 
%As long as the Euclidean projection\footnote{\todo{Could be generalize by proximal operators to solve sum of the LS with a non-smooth function}} operator is well-defined.
Also IPG (and more generally the proximal-gradient methods) has been considered to be particularly useful for big data applications \cite{Volkan:bigdata}\todo{or a better ref?}; It is memory efficient due to using only first order local oracles e.g., the gradient and the Euclidean projection onto $\Cc'$, it can be implemented in a distributed/parallel fashion, it is robust to using cheap statistical estimates, e.g. in stochastic descend methods\nref, to shortcut heavy gradient computations and as its rate of convergence is nearly independent of data size.


In this regard a major challenge that IPG encounters is the computational burden of performing an \emph{exact} projection step onto certain complex models. In many interesting inverse problems the model projection amounts to solving another optimization within each iteration. This includes important cases in practice such as the total variation penalized least squares \cite{Chambolle2011,TVprojGabirel}, lowrank matrix completion \cite{Ma2011} or tree sparse model-based CS \cite{modelbasedCS} to name a few. Another example is the convex inclusion constraints $\Cc'=\bigcap_i \Cc'_i$, appearing in \nref[spca][meLRJS], where one might be required to perform e.g. a Djkstra-type feasibility algorithm at each iteration\nref[combette pesqe].
In all these cases accessing to an exact oracle could be either computationally inefficient or even not possible (e.g. in analysis sparsity \nref), and therefore a natural line of thought is to carry those steps with cheaper \emph{approximate} oracles.

In this paper we feature an important property of the IPG algorithm; that \emph{it is robust against deterministic (worst case) errors in calculation of the projection and gradient steps.} 
We cover different types of oracles: i) A \emph{fixed precision} (FP) oracle which compared to the exact one has an additive bounded approximation error.  ii) A \emph{progressive fixed precision} (PFP) oracle which allows for larger (additive) approximations in the earlier iterations and refines the precision at an appropriate rate as the IPG iterations progress. iii) A $(1+\epsilon)$-approximate oracle which introduces a notion of relatively optimal approximation with a multiplicative error (as compared to the exact oracle). Our analysis uses a notion of model restricted bi-Lipschitz embedding similar as in e.g. \cite{Blumen}, however with improving the 
%(w.r.t. the forward operator $A$ and the signal model $\Cc'$)
%However improve the Blumensath's 
recovery condition in two folds: first by relaxing the purely uniform restrictions to a more local form which can avoid worst-case scenarios unnecessarily restricting the analysis, and second, by improving the requirement on the embedding conditioning by a factor (we discuss these in more details in Section X). With that respect, our analysis also slightly differentiates from the previous related works in convex settings as it enables us for instance to prove a globally optimal recovery result for nonconvex models, as well as establishing linear rate of convergences for the inexact IPG applied to the CS problems (e.g., results of \cite{BachinexactIPG} on linear convergence of the inexact IPG assumes strong convexity which does not hold in solving underdetermined least squares such as CS). In summary, we show that the FP type oracles restrict the final accuracy of the main reconstruction problem to be proportional to the approximation level introduced within each iteration. This limitation can be overcome by increasing the precision at an appropriate rate and one could achieve the same solution accuracy as for the exact IPG algorithm (and even within the same number of iterations) using the PFP type oracles. We show that the $(1+\epsilon)$-approximate projection can also achieve the accuracy of exact IPG however for moderately conditioned systems $A$ and using possibly more iterations (since using this type of oracle typically decreases the rate of convergence). In all cases above we study conditions that provide us with linear convergence results. Finally we study application of the inexact IPG  in data-driven compressed sensing problem. We shortcut the computations involved with (iteratively) performing exhaustive searches over large datasets by using approximate nearest neighbour search strategies corresponding to the aforementioned oracles and motivated by the cover tree structure introduced in \cite{beygelzimer2006cover}. By running several numerical experiments on a number of synthetic and real datasets we conclude similar observations as predicted by  our theoretical results.

The rest of this paper is organized as follows: In Section~\ref{sec:SOA} we review the previous related works on inexact IPG and compare our results/contributions to them. In Section~\ref{sec:prelim} we define the inexact IPG algorithm for three types of approximate oracles. Section~\ref{sec:main} includes our main theoretical bounds for robust CS recovery and linear convergence of the inexact IPG. %In this section we also define a hybrid (local-uniform) notion of bi-Lipschitz embeddingg.
We discuss an application of the proposed inexact IPG algorithms for data driven CS problems in Section~\ref{sec:datadrivenCS}. Section~\ref{sec:expe} is dedicated to the numerical experiments on using inexact IPG for data driven CS. 
And finally we discuss and conclude our results in Section XX\nref.

%This problem has been partly studied in both convex and nonconvex setting for which we provide more details in the next section. 

% This problem a.k.a. the \emph{inexact} IPG, has been studied in convex settings (and even for more general objectives than the CS problem under consideration here). A \emph{fixed precision} (FP) approximate oracles could be often obtained thanks to invoking the duality-gap information and stopping earlier the auxiliary optimization w.r.t. solving the projection. In this case the solution accuracy of the main  problem can not get better than the introduced approximation level. More recently \cite{BachinexactIPG} proposed and studied a \emph{progressive fixed precision} (FPF) type approximation scheme which refines the inexactness levels at an appropriate rate and achieves the same accuracy as for the exact IPG algorithm. However this result is only customized for convex problems and does not prove a linear convergence for CS related problems with non strong convexity.
%
%In nonconvex settings this has been tried for certain cases e.g. lowrank, tree-sparse, earth mover distance CS and by using $1+\epsilon$ type approximations.  This type of approximation introduces a notion of relatively optimal oracles with  a multiplicative error (as compared to the exact oracle).




%In this paper we show another important feature of IPG; that it is robust against deterministic (worst case) errors in calculation of the projection and gradient steps. This has straightforward implications \todo{e.g. for robust computation in distributed systems with errors}. However and of particular interest, this feature implies that one can  approximately conduct both steps to save in computations. For instance, this opens the possibility of using more complex models (which offer efficient representations for better CS reconstruction) with computationally exhaustive or even NP-hard projections, however approximable!







%. Moreover, we show that for certain decaying approximation errors, IPG solution maintain  the same accuracy as for the approximation-free (exact IPG) case.


%A general convergence result holds for both convex and non-convex constraints $\Cc'$, that is by choosing the step size small enough $\gamma\leq 1/\norm{A}$, IPGD converges to a critical point of the problem \eqref{eq:p1} which for convex $\Cc'$ is also a global convergence i.e., $\lim{x^{t}}\rightarrow x^{opt}$.  \nref ATOUCH. 
%
%Another class of results, guarantee near-optimal linear convergence of IPGD for non-convex $\Cc'$, when $A$ drawn at random from certain distributions (e.g. element-wise i.i.d. subgaussian, or random orthoprojector,...) and when number of the measurements $m > \dim(\Cc')$. \marginpar{can we be more regorous about dim here?} 


  


==> sections/mainresults1.tex <==
\section{Main results}
\label{sec:main}
\subsection{Uniform linear embeddings}
The success of CS paradigm relies heavily on 
%the low (intrinsic) dimensionality of most natural signals which can be captured by an efficient model, as well as 
the embedding property of certain random sampling matrices which preserves signal information for low dimensional but often complicated/combinatorial models. It has been shown that the exact IPG can stably predict the true signal $x^\gt$ from noisy CS measurements provided that $A$ satisfies the so called Restricted Isometry Property (RIP): 
\eql{\label{eq:RIP}(1-\theta)\norm{x-x'}^2 \leq \norm{A(x-x')}^2\leq (1+\theta)\norm{x-x'}^2, \quad \forall x,x' \in \Cc'
}
for a small constant  $0<\theta<1$.
This has been shown for models such as sparse, low-rank and low-dimensional smooth manifold signals and by using 
IPG type reconstruction 
algorithms which in the nonconvex settings are also known as Iterative Hard Thresholding \cite{IHTCS, Ma2011, AIHT,MIP, modelbasedCS}. Interestingly these results indicate that under the RIP condition (and without any assumption on the initialization) the first order IPG algorithms with cheap local oracles can globally solve
nonconvex optimization problems. 

For instance random orthoprojectors and i.i.d. subgaussian matrices $A$ satisfy RIP when the number of measurements $m$ is proportional to the intrinsic dimension of the model (i.e. signal sparsity level, rank of a data matrix or the dimension of a smooth signal manifold, see e.g. \cite{RichCSreview} for a review on comparing different CS models and their measurement complexities) and sublinearly scales with the ambient dimension $n$. 

A more recent work generalizes the theory of IPG to arbitrary \emph{bi-Lipschitz embeddable} models \cite{Blumen}, that is for given $\Cc'$ and $A$ it holds
\eq{\mm \norm{x-x'}^2\leq \norm{A(x-x')}^2\leq \MM \norm{x-x'}^2 \quad \forall x,x'\in \Cc'.}
for some constants $\mm, \MM >0$. Similar as for the RIP these constants are defined \emph{uniformly} over the constraint set i.e. $\forall x,x'\in \Cc'$. There Blumensath shows that if \eq{\MM<1.5\mm,} then IPG robustly solves the corresponding noisy CS reconstruction problem \emph{for all} $x^\gt\in \Cc'$. This result also relaxes the RIP requirement to a nonsymmetric and unnormalised notion of linear embedding whose implication in deriving sharper recovery bounds is previously studied by \cite{JaredJeff}. 

\subsection{Hybrid (local-uniform) linear embeddings}
Similarly the notion of restricted embedding plays a key role in our analysis. However we adopt a more local form of embedding and show that it is still able to guaranty stable CS reconstruction.  \marginpar{\todo{x0 or x*? C' deleted?}}

{\ass{ \label{def:Lip}
 Given $(x_0\in \Cc'\subseteq \Cc, A)$ there exists constants  $\MM,\mm_{x_0}>0$ for which the following inequalities hold:%\todo{$x_0$ or $x*$}
		%$A$ satisfies the following inequalities w.r.t. $\Cc$ and a point $x_0\in \Cc$:
		\begin{itemize}
			\item Uniform Upper Lipschitz Embedding (ULE)
			\begin{align*}
			\norm{A(x-x')}^2\leq \MM \norm{x-x'}^2 \quad \forall x,x'\in \Cc
			\end{align*}
			\item Local Lower Lipschitz Embedding (LLE)
			\begin{align*}
			\norm{A(x-x_0)}^2 \geq \mm_{x_0} \norm{x-x_0}^2 \quad \forall x\in \Cc
			\end{align*}
		\end{itemize}	
		Upon existence, $\MM$ and $\mm_{x_0}$ denote  respectively the smallest and largest constants for which the inequalities above hold.		
	}}
\newline
	
 Note that with respect to our distinction between the projection set $C$ and the original signal model $C'\subseteq C$ defined in \eqref{eq:proj1} and \eqref{eq:eproj}, our embedding assumption is on the projection set.
 
To compare with the previous results we shall set $\Cc=\Cc'$; which implies a weaker assumption compared to RIP or the uniform bi-Lipschitz embedding. Note that for any $x_0\in\Cc'$ and $\Cc=\Cc'$ we have: \eq{
\mm\leq\mm_{x_0}\leq\MM\leq \vertiii{A}^2
} 
(where $\vertiii{.}$ denotes the matrix spectral norm i.e. the largest singular value). 
In this case one has to sacrifice the \emph{universality} of the RIP dependant results for a signal $x^\gt$ dependent analysis. Depending on the study, local analysis could be very useful as for instance allows for avoiding worst-case scenarios that might unnecessarily restrict the recovery analysis~\cite{me:modelselecion}. In the convex settings it has been shown that local embeddings can improve the measurement bound and the speed of convergence up to sharp constants~\cite{recht:GW, Oymak:tradeoff}. 

Unfortunately we are currently unable to make the analysis fully local as we require the uniform RLS constraint. Nonetheless, one can always plug the stronger bi-Liptchitz assumption into our results throughout (i.e. replacing $\mmx$ with $\mm$) and regain the universality.  


%Our results on the exact and inexact FP approximate IPG improve the Blumensath's recovery condition in two folds: first by relaxing the uniform lower Lipschitz constant $\mm$ to a local form $\mmx$ which avoids worst-case scenarios that might unnecessarily restrict the recovery analysis (see Definition X), and second, by improving the factor in the Lipschitz embedding condition i.e. $\MM < 2\mmx$ for CS recovery (see e.g. Theorem 1). 






%In addition, if there exist a uniform constant $\mm>0$ such that 
%\eq{\mm\leq \mmx, \quad \forall x_0\in \Cc}
%then $A$ is a bi-Lipschitz embedding with constants $\mm,\MM$ i.e.
%\eq{\mm \norm{x-x'}^2\leq \norm{A(x-x')}^2\leq \MM \norm{x-x'}^2 \quad \forall x,x'\in \Cc.}
%Note that for any $x_0\in \Cc$ it holds \eq{\mm\leq\mm_{x_0}\leq\MM\leq \norm{A}^2.} 

%this assumption is weaker than  the so called Restricted Isometry Property (RIP) which guarantees performance of many CS reconstruction algorithms:
%{\defn{$A$ satisfies RIP w.r.t. a set $\Cc$ and a constant $0<\delta<1$, if $\forall x,x'\in \Cc$ it holds :
%		\eq{
%			(1-\delta)\norm{x-x'}^2\leq\norm{A(x-x')}^2\leq (1+\delta)\norm{x-x'}^2.
%			}
%}}
	
	
	
	

\subsection{Linear convergence of (P)FP inexact IPG for CS recovery}
In this section we show that IPG is robust against deterministic (worst case) errors. Moreover, we show that for certain decaying approximation errors, IPG solution maintain  the same accuracy as for the approximation-free (exact IPG) case.


In this part we assume neither $\ep^k$ or $\eg^k$ depend on $x^{k-1}$ or the previous updates.

{\thm{\label{th:inexactLS1} Assume $(x^\gt\in \Cc, \Cc,A)$ satisfy the main Lipschitz assumption  with constants $\MM< 2\mmx$. Set the step size $(2 \mmx )^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP} obeys the following bound:
		\eql{\label{eq:errbound}
			\norm{x^{k}-x^\gt}\leq  \rho^k \left(\norm{x^\gt}+\sum_{i=1}^k \rho^{-i} \nut^i \right)+ \frac{2\sqrt{\MM}}{\mmx(1-\rho)}w
		}
		where 
		\begin{align*}
		\rho=\sqrt{\frac{1}{\mu \mmx} -1} \qandq
		\nut^i=%\sum_{i=1}^k \rho^{-i}
		\frac{2\nug^i}{\mmx} + \sqrt{\frac{\nup^i}{\mu \mmx}},			
		\end{align*} 
		and $w=\norm{y-Ax^\gt}$.
	}} 

{\rem{Theorem \ref{th:inexactLS1} implications for the exact IPG (i.e. $\nup^k=\nug^k=0$) and inexact FP approximate IPG (i.e. $\nup^k=\nup,\nug^k=\nug, \forall k$)  improve  \cite[Theorem~2]{Blumen} in three folds: first by relaxing the uniform lower Lipschitz constant $\mm$ to a local form $\mmx\geq \mm$ and conduct a local recovery/convergence analysis. Second, by improving the embedding condition for CS stable recovery to 
\eql{\label{eq:cond}\MM < 2\mmx,
	} 
or $\MM < 2\mm$ for a uniform recovery $\forall x^\gt\in\Cc$. And third, by improving  twice faster the rate $\rho$ of convergence.}}

The following corollary is an immediate consequence of linear convergence established in Theorem \ref{th:inexactLS1} for which we do not provide proof:
{\cor{\label{cor:FP}With assumptions in Theorem \ref{th:inexactLS1} the IPG algorithm with FP approximate oracles achieves the solution accuracy
\eq{\norm{x^K-x^\gt}\leq 
		 	\frac{1}{1-\rho}\left(\frac{2\nug}{\mmx} + \sqrt{\frac{\nup}{\mu \mmx}},+ \frac{2\sqrt{\MM}}{\mmx}w\right) +\tau}
for a $\tau>0$ and in a finite number of iterations
\eq{
	K=\left\lceil\frac{1}{\log(\rho^{-1})} \log\left( \frac{ \norm{x^\gt}}{\tau}\right)\right\rceil
	}			
}}
As it turns out in our experiments and aligned with the result of Corollary~\ref{cor:FP}, the solution accuracy of IPG can not exceed the precision levels introduced by PF oracles. In this sense Corollary~\ref{cor:FP} is tight as a trivial converse example would be that IPG starts from the optimal solution $x^\gt$ but an adversarial FP scheme projects it to another point within a fixed distance. 

Interestingly one can make another implication of Theorem~\ref{th:inexactLS1} and overcome such limitation using the PFP type oracles.
%Here comes 
%an interesting part of Theorem \ref{th:inexactLS1} analysing the behaviour of the PFP type oracles. 
Remarkably 
one achieves a linear convergence to a solution with the same accuracy as for the exact IPG, 
as long as $\nut^k$ geometrically decays. 	
The following corollary makes this statement explicit:
	
%{\cor{\label{cor:decay}Assume $\nut^k= O(r^k)$ for some error decay rate $0<r<1$ and a constant $C$. We have 
%			%After a finite number $k\geq K$ of iterations 
%			\eq{
%				\norm{x^{k}-x^*}\leq %\rho^k \norm{x^0-x'} +
%				\frac{2\sqrt{\MM}}{\mm_{x^\gt}(1-\rho)} w+ O({\bar \rho}^k), 
%			}
%			where $\rho$ is the same as in Theorem \ref{th:inexactLS1}, and
%			\begin{align*}
%			%&x^\rsc_{\min}\in \argmin_{x^\rsc\in \Omega}\norm{\nabla f(x^\rsc)},\\
%			%&K=\left\lceil\log\left( \frac{2\norm{\nabla f(x^\rsc_{\min})}}{m(1-\rho) \norm{x^\rsc_{\min}}}\right)/\log(\bar \rho)\right\rceil,\\
%			\bar \rho = \choice{\max(\rho,r)\quad r\neq\rho \\
%				r+\xi\qquad\quad r=\rho}
%			\end{align*}
%			for an arbitrary small $\xi>0$.	
%}
%}
	
{\cor{\label{cor:decay}Assume $\nut^k\leq Cr^k$ for some error decay rate $0<r<1$ and a constant $C$. Under the assumptions of Theorem~\ref{th:inexactLS1} the solution updates $\norm{x^{k}-x^*}$ of the IPG algorithm with PFP approximate oracles is bounded above by:
		%After a finite number $k\geq K$ of iterations 
		\begin{align*}
			%\norm{x^{k}-x^*}\leq 
			&\max(\rho,r)^k \left(\norm{x^\gt}+\frac{C}{1-\frac{\min(\rho,r)}{\max(\rho,r)}}\right) +
			\frac{2\sqrt{\MM}}{\mm_{x^\gt}(1-\rho)} w,  &r\neq \rho \\
			&\rho^k \Big(\norm{x^\gt}+Ck\Big) +
			\frac{2\sqrt{\MM}}{\mm_{x^\gt}(1-\rho)} w, &r=\rho 
		\end{align*}
		Which implies a linear convergence at rate 
%		$\bar \rho$:
%		\eq{
%		\norm{x^{k}-x^*}\leq %\rho^k \norm{x^0-x'} +
%		\frac{2\sqrt{\MM}}{\mm_{x^\gt}(1-\rho)} w+ O({\bar \rho}^k), 
%		}
%		where,
		\begin{align*}
		%&x^\rsc_{\min}\in \argmin_{x^\rsc\in \Omega}\norm{\nabla f(x^\rsc)},\\
		%&K=\left\lceil\log\left( \frac{2\norm{\nabla f(x^\rsc_{\min})}}{m(1-\rho) \norm{x^\rsc_{\min}}}\right)/\log(\bar \rho)\right\rceil,\\
		\bar \rho = \choice{\max(\rho,r)\quad r\neq\rho \\
			\rho+\xi\qquad\quad r=\rho}
		\end{align*}
		for an arbitrary small $\xi>0$.	
	}
}
{\rem{Similar to Corollary \ref{cor:FP} 
%and due to the linear convergence 
one can increase the final solution precision of the FPF type  IPG with logarithmically more iterations i.e. in a finite number $K=O(\log(\tau^{-1}))$ of iterations one achieves $\norm{x^{k}-x^*}\leq O(w)+\tau$. As we can see (and in contrast with the FP oracles) one could achieve an accuracy within the noise level $O(w)$ that is the precision of an approximate-free IPG.
}}

{\rem{Using the PFP type oracles can also maintain the rate of linear convergence identical as for the exact IPG. For this the approximation errors suffice to follow a geometric decaying rate of  $r<\rho$. \todo{discuss suitable oracle complexity within PFP.}
}}

\subsection{Linear convergence of inexact IPG with $(1+\epsilon)$-approximate projection for CS recovery}
\label{sec:relative}
In this part we focus on analysing the inexact IPG algorithm with a $(1+\epsilon)$-approximate projection. As it turns out in the following theorem we require a stronger condition on the embedding to guaranty the CS stability as compared to that \eqref{eq:cond} for the previous cases.
%the exact or the FP/PFP type inexact IPG. 


{\thm{\label{th:inexactLS2} Assume $(x^\gt\in \Cc, \Cc,A)$ satisfy the main Lipschitz assumption and that
		\eq{\sqrt{\epsilon+\epsilon^2}\leq \delta\frac{\sqrt{\mmx}}{\vertiii{A}} \qandq \MM < (2-2\delta+\delta^2) \mmx} 	
		for $\epsilon\geq 0$ and some constant $\delta \in [0,1)$.
		Set the step size $\left((2-2\delta+\delta^2) \mmx\right)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP2} obeys the following bound:
		\eq{
			\norm{x^{k}-x^\gt}\leq  \rho^k \left(\norm{x^\gt}+\kappa_g \sum_{i=1}^k \rho^{-i} \nug^i \right)+ 
			%\frac{ \left( 2\frac{\sqrt{M}}{m}+\frac{\sqrt\mu}{\norm{A}}\delta \right)}
			\frac{\kappa_w}{1-\rho}w
		}
		where 
		\begin{align*}
		&\rho=\sqrt{\frac{1}{\mu \mmx} -1}+ \delta, \quad
		\kappa_g = \frac{2}{\mmx}+\frac{\sqrt\mu}{\vertiii{A}}\delta, \\		
		&\kappa_w= 2\frac{\sqrt{\MM}}{\mmx}+\sqrt\mu\delta, \qandq w=\norm{y-Ax^\gt}.
		\end{align*}		
		
	}} 	
{\rem{Similar conclusions can be made as in Cor1,2 on the linear convergence, logarithmic number of iterations vs final level of accuracy (depending whether the gradient oracle is exact or FP/PFP) however with a stronger requirement than \eqref{eq:cond} on the embedding: increasing $\epsilon$ limits the recovery guaranty and slows down the convergence (by comparing $\rho$ in Theorems 1 and 2) as $\epsilon$ increases.}}

{\rem{Assumptions of Theorem \ref{th:inexactLS2} impose a stringent requirement on the scaling of the approximation parameter i.e. $\epsilon=O\left(\sqrt{\frac{\mmx}{\vertiii{A}}}\right)$ which is not purely dependant to the model restricted embedding conditioning but also the spectral norm of $\vertiii{A}$. In this sense since  $\vertiii{A}$ ignores the structure $\Cc$ of the problem it might scale very differently as compared to the corresponding embedding constants $\mmx,\mm$ and $\MM$. For instance an $m\times n$  i.i.d. Gaussian matrix have with high probability $\vertiii{A}=\Theta(n)$ (when $m\ll n$) whereas, e.g. for $s$-sparse signals, its embedding constants $\mm,\MM$ w.h.p. scale as $O(m)$. A similar gap exists for other low dimensional signal models and for other compressed sensing matrices e.g. random orthoprojectors, 
%for$(s\ll m)$ sufficiently large $m$ hav This is the case for e.g. orthoprojectors and subgaussians matrices often 
which is unfavourable for applying large approximation of this type to the extreme compressed sensing settings where $\sqrt{\frac{\mmx}{\vertiii{A}}}\approx \sqrt{\frac{m}{n}}\rightarrow 0$. 
}}

In the following we show by a deterministic example that this requirement is indeed tight. We also observe empirically in Section \ref{sec:expe} that such limitation indeed holds in randomized settings (e.g. i.i.d. Gaussian $A$) and on average. 

\subsubsection*{A converse example}
Consider a noiseless CS recovery problem where $n =2$, $m=1$ and the sampling matrix (i.e. here a row vector) is
\eq{A=[\cos(\gamma)\quad -\sin(\gamma)]}
for some parameter $0\leq\gamma\leq\pi/2$. Consider the following signal model which is a line segment across the first dimension:
\eq{
\Cc = \{x\in \RR^2: 0\leq x(1)\leq 1,\, x(2)=0\}.
}
We have indeed $\vertiii{A}=1$. It is easy to verify that both of the embedding constants w.r.t. to $\Cc$ are
\eq{ \mmx=\MM = \cos(\gamma)^2.}
Therefore one can tune $\gamma\rightarrow \pi/2$ to obtain arbitrary small ratios for $\sqrt{\frac{\mmx}{\vertiii{A}}}=\cos(\gamma)$. 
%$\vertiii{A}$ and $\mmx$ the 

Assume the true signal and the initialization point are at the either ends of $\Cc$ i.e.
\eq{
x^\gt=[1 \quad 0]^T,\quad y=Ax^\gt=\cos(\beta) \qandq x^0=[0 \quad 0]^T.
}
%and the initialization point $x^0=(0,0)^T$. 
Consider an adversarial $(1+\epsilon)$-approximate projection oracle which performs the following step for any given $x\in \RR^2$: \marginpar{\todo{verify + this part modified $\epsilon$}}
\eq{
		\pp_\Cc^{\epsilon}(x) := [x(1)+\epsilon x(2) \quad 0]^T.
	}
For simplicity we assume no errors on the gradient step. 	
By setting $\mu=1/\cos(\gamma)^2$, the corresponding inexact IPG updates as 
\eq{	
	x^k(1)= \epsilon\tan(\gamma) \left(x^{k-1}(1)-1\right) + 1 
}
and only along the first dimension (we note that due to the choice of oracle $x^k(2)=0, \forall k$). Therefore
\eq{	
	x^k(1)= \left(\epsilon\tan(\gamma)\right)^k+1.
}
which requires $\epsilon<\tan^{-1}(\gamma)=O(\cos(\gamma))$ for convergence, and it diverges otherwise. As we can see for $\gamma\rightarrow \pi/2$  (i.e. where $A$ becomes extremely unstable w.r.t. sampling the first dimension) the range of admissible $\epsilon$ shrinks, irrespective of the fact that the restricted embedding $\mmx=\MM$ exhibits an perfect isometry; which is an ideal situation for solving a noiseless CS with the exact IPG (i.e. in this case IPG takes only one iteration to converge).




==> sections/setup1.tex <==
\section{Preliminaries}\label{sec:prelim}
Iterative projected gradient iterates between calculating the gradient and projection onto the model 
i.e. for positive integers $k$ the \emph{exact} form of IPG follows:
\eql{\label{eq:IP}
	x^{k} = \pp_{\Cc'}\left(x^{k-1}-\mu \nabla f(x^{k-1})\right) }
where, $\nabla f(x)=A^T(Ax-y)$ and $\pp_\Cc'$ denote the exact gradient and the Euclidean projection oracles, respectively.  We do not make a particular assumption on  the initialization and we set $x^0=\mathbf{0}$ throughout (also for the inexact form of IPG which we shall define next). The exact IPG requires   
%problem \eqref{eq:p1} has solution(s) and	
the constraint set $\Cc'$ 
 to have a well defined, not necessarily unique but  computationally tractable Euclidean projection $\pp_{\Cc'}:\RR^n\rightarrow \Cc'$ 
% \footnote{Closeness of $\Cc$ %and a lower bound on $f$ 
% 	implies the existence of such minimum i.e. the exact projection. %$x^*$ for \eqref{eq:p1}. 
% 	%One might drop the closeness condition but rather use a FP type approximate projection as discussed in \cite{Blumen}.
% 	}:
\eq{
	\pp_{\Cc'}(x)\in \argmin_{u\in\Cc'}\norm{u-x}.}
Throughout we use $\norm{.}$ as a shorthand for  the Euclidean norm $\norm{.}_{\ell_2}$. 
%Closeness of $\Cc'$ 
%implies the existence of a minimum, however we do not assume uniqueness for the exact projection. 

In the following we define three types of approximate oracles which frequently appear in the literature and could be incorporated within the IPG iterations. We also briefly discuss their applications. 
\newline
\textbf{Important note:} We incorporate throughout the flexibility of considering an approximate projection onto a (possibly) larger set $C$ including the original signal model $x^\gt \in C'\subseteq C$ , which for instance finds practical implications in tree-sparse signal or lowrank matrix CS recovery, see \cite{HegdeISIT,MatrixAlpsapprox}.
\subsection{Fixed Precision (FP) approximate oracles}
\label{sec:FP}
We first consider 
%fixed precision (FP) 
approximate oracles with \emph{additive} bounded-norm 
%varying 
errors, namely the fixed precision gradient oracle $\nablaa^{\nug} f(x):\RR^n\rightarrow \RR^n$ where:
\begin{align}
\norm{\nablaa^{\nug} f(x) -\nabla f(x)}\leq \nug, \label{eq:grad} 
\end{align}
and the fixed precision projection oracle $\pp_\Cc^{\nup}:\RR^n\rightarrow\Cc$ where:
\begin{align}
\pp_\Cc^{\nup}(x) \in \Big\{ u\in \Cc :\,	\norm{u-x}^2 \leq \inf_{u'\in \Cc'}\norm{u'-x}^2 +\nup  \Big\}.\label{eq:proj1}
\end{align} 
The values of $\nug,\nup$ denote the levels of inaccuracy in calculating the gradient and projection steps respectively. 
The corresponding \emph{inexact} IPG
%for the gradient IPG with a fixed-precision accuracy 
iterates as follows:
%\eql{\label{eq:inIP} x^k = \pp^{\nup^k}_{\Cc}\left(x^{k-1}-\mu( \nabla f(x^{k-1}) + \eg^k)\right) + \ep^k.}
\eql{\label{eq:inIP} x^k = \pp^{\nup^k}_{\Cc}\left(x^{k-1}
	%-\mu\left( \nabla f(x^{k-1}) + \eg^k\right)\right), }	
-\mu \nablaa^{\nug^k} f(x^{k-1})\right).}
Note that in this formulation we allow for variations in the inexactness levels at different stages of IPG. % \todo{however we assume neither $\ep^k$ or $\eg^k$ depend on $x^{k-1}$ or the previous solution updates.}  
The case where the accuracy levels are bounded by a constant threshold $\nup^k=\nup$ and $\nug^k=\nug$, $\forall k$, refers to an inexact IPG algorithm with \emph{fixed precision} (FP) approximate oracles.

% which could apply for instance in  distributed network

%In this regard a \emph{Fixed precision} (FP) inexact IPG refers to having approximate oracles with accuracy levels bounded by a constant threshold i.e.  $\nup^k=\nup$ and $\nug^k=\nug$, $\forall k$. 
\subsubsection*{Examples}
Such errors can occur for instance in distributed network
optimizations where the gradient calculations could be noisy during the communication on the network\nref[.], or in CS under UoS models with infinite subspaces \cite{Blumen} where an exact projection might not exist by definition when e.g. $\Cc=\Cc'$ is an open set, however a FP type approximation could be achievable. It also has application in finite super resolution\nref, source localization and separation \cite{TASL14,SCOOP}, and data driven CS problems e.g., in Magnetic Resonance Fingerprinting \cite{MRF,BLIPsiam},  where typically a continuous manifold is first discretized into a finite precision and large dictionary which is eventually used for e.g. sparse recovery.\todo{but this is $C\subseteq C'$?}
\subsection{Progressive Fixed Precision (PFP) approximate oracles}\label{sec:PFP}
One obtains a \emph{Progressive Fixed Precision} (PFP) approximate IPG algorithm by refining the FP type precisions thorough the course of iterations. Therefore any FP gradient or projection oracle which has control on tuning its accuracy could be used in this setting and follows \eqref{eq:inIP} with decaying sequences $\nup^k,\nug^k$.
\subsubsection*{Examples}
For instance this case includes projection schemes which require iteratively solving an auxiliary optimization (e.g. the total variation ball \cite{TVprojGabirel}, sparse CUR factorization \cite{BachinexactIPG} or the multi-constraint inclusions\nref, etc) and can progress (at an appropriate rate) on the accuracy of their solutions by adding more subiterations. We also discuss in Section~\ref{sec:covertree} another example 
%of the PFP type projection oracles 
in this form that is customized for fast approximate nearest neighbour searches and its 
application to the data driven CS framework.

\subsection{$(1+\epsilon)$-approximate projection}\label{sec:epsproj}
For some constraint sets obtaining a fixed precision (and thus PFP) accuracy in projections might be still computationally exhaustive, whereas a notion of relative optimality 
%oracles with multiplicative errors are 
could be more efficient to implement. The $(1+\epsilon)$-approximate projection is defined as follows and for a given $\epsilon\geq0$:
\eql{\label{eq:eproj}
	\pp_\Cc^{\epsilon}(x) \in \Big\{ u\in \Cc :\,	\norm{u-x} \leq (1+\epsilon)\inf_{u'\in \Cc'}\norm{u'-x}  \Big\}. 
}
We note that $\pp_\Cc^{\epsilon}(x)$ might not be unique. In this regard, the inexact IPG algorithm with a $(1+\epsilon)$-approximate projection takes the following form:
\eql{\label{eq:inIP2}
	x^k = \pp_\Cc^{\epsilon}\left(x^{k-1}
	%-\mu( \nabla f(x^{k-1}) + \eg^k)\right).
	-\mu \nablaa^{\nug^k} f(x^{k-1})\right).}
Note that we still assume a fixed precision gradient oracle with flexible accuracies $\nug^k$.  
%$\norm{\eg^k}\leq \nug^k$. 
One could also consider a $(1+\epsilon)$-approximate gradient oracle and in combination with those aforementioned inexact projections however for brevity and since the analysis is quite  similar to the relative approximate projection case we skip more details on this case (one might be able to link this with d'aspremond works on subselecting row of $A$ for implementing cheaper statistical gradients).  
\subsubsection*{Examples}
The tree $s$-sparse projection in $\RR^n$ and in the exact form requires solving a dynamical programming with $O(ns)$ running time \cite{DRthompson} whereas solving this problem approximately with $1+\epsilon$ accuracy requires the time complexity of $O(n\log(n))$ \cite{HegdeISIT} which suits better most imaging problems in practice with a Wavelet sparsity level of typically $s=\Omega(\log(n))$. Also \cite{StoIHT,MatrixAlpsapprox} show one can reduce the cost of lowrank matrix completion problem by using randomized linear algebra methods, e.g. see \cite{Deshpande2006,HalkoTropp}, and carry out fast lowrank factorizations with a $1+\epsilon$ type approximation. \todo{can we say something here about submodular optimization [Krause] with greedy algos and their 1+e guaranty?}
We also discuss in Section~\ref{sec:covertree} another example 
%of the PFP type projection oracles 
in this form that is customized for fast approximate nearest neighbour searches and its 
application to the data driven CS framework.


%In a similar fashion the fixed precision (FP) approximate projection oracle is defined:

 

 
%It has been shown that under certain conditions and for a well chosen step size $\mu$ IPG converges to a solution of \eqref{eq:p1}.


